Distilling Text into Circuits

This paper concerns the structure of meanings within natural language. Earlier, a framework named DisCoCirc was sketched that (1) is compositional and distributional (a.k.a. vectorial); (2) applies to general text; (3) captures linguistic `connections' between meanings (cf. grammar) (4) updates word meanings as text progresses; (5) structures sentence types; (6) accommodates ambiguity. Here, we realise DisCoCirc for a substantial fragment of English. When passing to DisCoCirc's text circuits, some `grammatical bureaucracy' is eliminated, that is, DisCoCirc displays a significant degree of (7) inter- and intra-language independence. That is, e.g., independence from word-order conventions that differ across languages, and independence from choices like many short sentences vs. few long sentences. This inter-language independence means our text circuits should carry over to other languages, unlike the language-specific typings of categorial grammars. Hence, text circuits are a lean structure for the `actual substance of text', that is, the inner-workings of meanings within text across several layers of expressiveness (cf. words, sentences, text), and may capture that what is truly universal beneath grammar. The elimination of grammatical bureaucracy also explains why DisCoCirc: (8) applies beyond language, e.g. to spatial, visual and other cognitive modes. While humans could not verbally communicate in terms of text circuits, machines can. We first define a `hybrid grammar' for a fragment of English, i.e. a purpose-built, minimal grammatical formalism needed to obtain text circuits. We then detail a translation process such that all text generated by this grammar yields a text circuit. Conversely, for any text circuit obtained by freely composing the generators, there exists a text (with hybrid grammar) that gives rise to it. Hence: (9) text circuits are generative for text.

==> rules.tex <==
\clearpage
\section{Language Circuit Conventions and Lexical Assumptions}
\paragraph{We assume all verbs come with passive forms that change argument order}
\[\tikzfig{passiveconvention}\]
\paragraph{We assume all higher-order verbs are synthetic}
\[\tikzfig{DVconvention}\]
\paragraph{We assume the presence of reflexive pronoun boxes}
\[\tikzfig{selfbox}\]
\paragraph{We assume the verb \texttt{EXISTS}}
\[\tikzfig{exists}\]
And the copular \texttt{IS} for cases where a noun wire only has adjective gates.

\clearpage
\section{Grammatical Diagrams}
We omit the labelling rules.
\subsection{``Phrase Structure" component}
Any diagram made of these generators gives a planar Grammatical Diagram.
\paragraph{Initial States}
\[\tikzfig{123wire}\]
\paragraph{Verbs}
\[\tikzfig{IVgate} \quad\quad \tikzfig{TVgate} \quad\quad \tikzfig{SCVbox}\]

\paragraph{Modifiers}
\[\tikzfig{ADJgate} \quad\quad \tikzfig{ADVIVbox} \quad\quad \tikzfig{ADVTV} \quad\quad \tikzfig{ADPIVbox} \quad\quad \tikzfig{ADPTVbox}\]
\paragraph{Conjunctions}
\[\tikzfig{CNJbox}\]
\paragraph{Phrase Scope}
\[\tikzfig{phrenter} \quad\quad \tikzfig{phrexit} \quad\quad \tikzfig{phrenterR} \quad\quad \tikzfig{phrexitR} \quad\quad \tikzfig{phrcap}\]
We have omitted here and in paper the modifiers for verbs with a sentential complement, but their structure and reduction rules to gates are straightforward.

\paragraph{Pronominal Links}
Pronominal links, depicted grey and dotted, are allowed to freely cross wires of all other types.
\[\tikzfig{plinkgens}\]

\paragraph{Special Pronominal Constructions}
$\texttt{VP}$s denote Grammatical Diagrams with a single verb gate. $\texttt{NP}$s denote Grammatical Diagrams with no verb gates.

\[\tikzfig{subrelpron} \quad\quad \tikzfig{subrelpronspec} \]
\[\tikzfig{obrelpron} \quad\quad \tikzfig{reflpron}\]

\subsection{``Transformational" component}
$\mathcal{C}$ denotes an arbitrary circuit. Rules are parameterised by all labels.
\paragraph{Verbs to Gates}
\[\tikzfig{IVredux} \quad\quad \tikzfig{TVredux} \quad\quad \tikzfig{SCVredux}\]
\paragraph{Adjectives}
\[\tikzfig{ADJredux} \quad\quad \tikzfig{ADJistransform}\]
\paragraph{Modified Verbs to Gates}
\[\tikzfig{ADVredux} \quad\quad \tikzfig{ADVTVredux}\]
\[\tikzfig{ADPIVredux} \quad\quad \tikzfig{ADPTVredux}\]
\paragraph{Conjunctions}
\[\tikzfig{CNJredux}\]
\subsubsection{Pronominal Link Handling}
\paragraph{Pronominal Link Introduction and Elimination}
\[\tikzfig{pronlinkrule} \quad\quad\quad\quad \tikzfig{pronlinkrule2}\]
\subsection{Gate Normal Form}
\paragraph{Definition}
A grammatical diagram $\Gamma$ is in GNF just when:
\begin{itemize}
    \item not counting pronominal links, $\Gamma$ is a collection of disjoint, side-by-side diagrams $\texttt{VP}_{i \in I}$
    \item each $\texttt{VP}$ diagram corresponds to a single gate in circuit form.
    \item pairs of wires may be pronominally linked, but each pair at most once, and not in a cycle.
\end{itemize}

==> snippets.tex <==
\subsection{Reading off language circuits}

Language circuits can be turned back into sentences (not necessarily in a unique way) as follows. We adopt the following conventions to do so:

We regard the empty wire as a valid gate, corresponding to the special intransitive verb \texttt{exists}.
\[\tikzfig{tikzfigs/exists}\]

Further, we gloss parallel composition as the conjunction \texttt{while}, and sequential composition as the comma punctuation \texttt{,}

So, starting from a language circuit:
\[\tikzfig{tikzfigs/circtosentex1}\]
We use the sliding rules defined in the previous section to obtain horizontal slices, where all gates on each horizontal slice are composed in parallel, and recursing the process in boxes. This obtains, for instance:
\[\tikzfig{tikzfigs/circtosentex2}\]

Which we can then read off as:
\texttt{A sees B likes F that C picks while D hates E, A\&B\&F\&C\&D exist while E runs quickly}

The question is now to precisely characterise the behaviour of such grammatical words as the relative pronoun \texttt{that} and \texttt{\&}, in terms of composition instructions for circuits. Then there is the matter of determining a grammar for a language consisting of the lexicon and these grammatical words, and proving a correspondence between circuits and sentences of this grammar.
